Automatic Synthesis of Switching Controllers for Linear Hybrid Automata

In this paper we study the problem of automatically generating switching controllers for the class of Linear Hybrid Automata, with respect to safety objectives. We identify and solve inaccuracies contained in previous characterizations of the problem, providing a sound and complete symbolic fixpoint procedure, based on polyhedral abstractions of the state space. We also prove the termination of each iteration of the procedure. Some promising experimental results are presented, based on an implementation of the fixpoint procedure on top of the tool PHAVer.

==> reachability.tex <==
\section{Reachability Control} \label{sec:reach}

\subsection{The Abstract Algorithm}

\paragraph{Fixpoint algorithm.}
The answer to the reachability control problem for target set $T\subseteq\Invs$
is positive if and ony if
$$
\Inits \subseteq \mu W \qdot T \cup \cpre^R(W),
$$
where $\cpre^R$ is the controllable predecessor operator for reachability,
defined in the following section.


\paragraph{Controllable predecessor operator.}
For a set of states $A$, the operator $\cpre^R(A)$ returns the set of states
from which the controller can ensure that the system reaches $A$
in the next joint transition.
This may happen for two reasons: first, without issuing any controllable
transition, the system may naturally reach $A$ via continuous evolution
or uncontrollable transitions; second, a controllable transition will
lead to $A$, and any uncontrollable transition that may happen before
also leads to $A$. 
%
Formally, we have:
%
\begin{align*}
\cpre^R(A) = &\Bigl\{ p \in S \,\Bigl|\, \forall f \in \adm(p) \,
\exists \delta \geq 0:\\
&\text{either } \exists p'\in A : p \xrightarrow{\delta, f} p'
\text{ and } p\in\while(S,A,f,\delta)\\
&\text{or } \exists e \in \edg_c, \, p' \in A :
p \xrightarrow{\delta, f, e} p' \text{ and }  p\in\while(S,A,f,\delta) \Bigr\}.
\end{align*}


\subsection{Computing the Predecessor Operator} %\label{sec:compute-reach}

In order to compute the predecessor operator, we introduce another version
of the $\rwamay$ operator, denoted by $\rwamust$: Must Reach While Avoiding.
Given a location $l$ and two sets of variable valuations $U$ and $V$,
$\rwamust_l(U,V)$ contains the set of valuations
from which the continuous evolution of the system \emph{must} reach $U$
while avoiding $V$~\footnote{In $\atl$ notation,
we have $\rwamust(U,V) \equiv \team{ctr} \overline{V} \U (U \wedge \overline{V})$,
where $ctr$ is the player representing the controller.}.
%
Formally, we have:
\begin{multline*}
\rwamust_l(U, V) = \Bigl\{ u \in \Val(X) \,\Bigl|\,
\forall f\in\adm(\pair{l,u}) \, \exists \delta\geq 0: \\
f(\delta)\in U \text{ and }
\forall\, 0 \leq \delta'\leq\delta: f(\delta')\not\in V \Bigr\}.
\end{multline*}
%
Notice that $\rwamust$ differs from $\rwamay$ only on the quantification of
the activity $f$ and on the inequality $\delta'\leq\delta$, which is strict
in $\rwamay$. The latter difference is connected to the fact that the controller
must prevent ``bad'' uncontrollable transitions
even if they occur at the same time as a ``good'' controllable transitions.
This connection is exploited in the proof of the following Lemma,
which states the relationship between $\cpre^R$ and $\rwamust$.
%
\begin{lemma}\label{lem:Rcpre}
For all sets of states $A \subseteq \Invs$, we have
$$ \cpre^R(A) = \bigcup_{l \in \Loc} \{ l \} \times 
\rwamust_l \big( \proj{A}{l} \cup C_l, B_l \cup
\overline{\proj{\Invs}{l}} \big) \,,$$
%~\footnote{TO FIX: dalla
%  definizione di $\cpre^R$ sembra che un punto in $A_l\cap B_l$ non
%  appartenga al $\cpre^R(A)$. Dovrebbe bastare:
%$$ \cpre^R(A) = \bigcup_{l \in \Loc} \{ l \} \times \rwamust_l
%  \big(\proj{A}{l} \cup C_l, B_l \cup \overline{\proj{\Inv}{l}} \big)
%  \,,$$ }
where $B_l$ and $C_l$ are defined as in~\eqref{eq:BC}.
\end{lemma}
\begin{proof} The thesis immediately follows from the definitions of $\cpre^R(A)$, 
$\rwamust_l$, $C_l$ and $B_l$.
\end{proof}

\subsection{Computing the $\rwamust$ Operator} %\label{sec:compute-reach}

We show how to compute $\rwamust$ based on $\rwamay$, plus a simple
preliminary step. In this section, we consider a fixed location $l \in
\Loc$.\\ For a (not necessarily convex) polyhedron $G$ and a convex
polyhedron $F$, we say that $G$ is \emph{bounded w.r.t.\ $F$} if for
all $p \in G$ and all $c \in F$ there exists a constant $\delta\geq 0$
such that $p + \delta c \not\in G$.  Moreover, we say that $G$ is
\emph{thin w.r.t.\ $F$} if for all $p \in G$, $c \in F$, and $\delta >
0$, it holds $p + \delta c \not\in G$.  Intuitively, $G$ is bounded
(resp., thin) w.r.t.\ $F$ if all straight lines starting from $G$ and
whose slope belongs to $F$ eventually (resp., immediately) exit from
$G$.  Obviously, being thin w.r.t.\ $F$ implies being bounded
w.r.t.\ $F$.
%
We denote by $\origin$ the origin, i.e., the point whose coordinates are $0$.
%Given a polyhedron $G$ and a convex polyhedron $F$,
%we introduce the \emph{positive pre-flow} operator $\pospref{G}F$:
%$$
%\pospref{G}F = \{ u \in \Val(X) \mid \exists c\in F, \delta>0 : 
%p + \delta \cdot c \in G \}.
%$$
%%
The following is a trivial observation.
%
\begin{proposition} \label{prop:origin-in}
If $F$ is a convex polyhedron containing the origin,
no polyhedron is bounded w.r.t.\ $F$.
\end{proposition}
%
Additionally, given $p \in G$, we say that $p$ is 
\emph{$l$-bounded in $G$} (resp., \emph{$l$-thin in $G$})
if all admissible activities
starting from $p$ eventually (resp., immediately) exit from $G$.
Formally, $p$ is $l$-bounded if for all $f \in\adm(\pair{l,p})$
there exists $\delta\geq 0$ such that $f(\delta) \not\in G$;
$p$ is $l$-thin if for all $f \in\adm(\pair{l,p})$
and all $\delta > 0$, it holds $f(\delta) \not\in G$.
We denote by $\bounded_l(G)$ the set of points of $G$ 
that are $l$-bounded in it,
and we say that $G$ is \emph{$l$-bounded} (resp., \emph{$l$-thin})
if all points $p\in G$ are $l$-bounded (resp., $l$-thin) in $G$.
It is easy to verify that a polyhedron is $l$-thin if and only
if it is thin w.r.t.\ $\Flow(l)$.
%
The following results explore the relationship between (geometric) boundedness
and $l$-boundedness.
%
\begin{lemma} \label{lem:easy}
If a polyhedron is $l$-bounded, then it is bounded w.r.t.\ $\Flow(l)$.
\end{lemma}
%
It is easy to verify that being bounded w.r.t.\ $\Flow(l)$ is necessary
but not sufficient for a polyhedron to be $l$-bounded.
Lemma~\ref{lem:exit1} shows a sufficient condition; namely,
that if a polyhedron is bounded w.r.t.\ the topological closure of $\Flow(l)$,
then it is also $l$-bounded.
First, we show that if the origin does not belong to the topological
closure of the flow, then there is a flow direction $u$ such that all
possible flows advance in the direction $u$ 
by at least $|u|$ for each time unit.
%
\begin{lemma} \label{lem:origin-out}
If $\origin \not\in \clos{\Flow(l)}$ 
then there exists $u \in \clos{F}$ such that for all $v \in F$
the scalar projection of $v$ onto $u$ is at least $|u|$
(i.e., $\frac{u \cdot v}{|u|} \geq |u|$, where $\cdot$ denotes the inner product).
\end{lemma}

\begin{lemma} \label{lem:exit1}
If a polyhedron is bounded w.r.t.\ $\clos{\Flow(l)}$
then it is $l$-bounded.
\end{lemma}
%
We can now state the main result of this section.
% Moreover, if activities were not necessarily
%Lipschitz continuous, the result would also fail.

\begin{theorem} \label{thm:must}
Let $\over$ be a polyhedron such that \emph{(i)} $\over$ is $l$-bounded,
and \emph{(ii)} $\rwamust_l(U,V) \subseteq (U\setminus V) \cup \over$.
Then,
\begin{equation} \label{eq:must}
\rwamust_l(U,V) =  (U \setminus V) \cup
(\over \setminus \rwamay_l(\overline{\over}\cup V, U)).
\end{equation}
\end{theorem}

Theorem~\ref{thm:must} leaves us with one last problem. We need to be
able to compute a $l$-bounded polyhedron $\over$ satistyng condition
\emph{(ii)} of the theorem. In order to show that such a polyhedron
can easily be computed, we first need to introduce an additional
operatator.  Given a polyhedron $G$ and a convex polyhedron $F$, the
\emph{positive pre-flow} operator $\pospref{G}F$ is defined as
follows:
$$
\pospref{G}F = \{ u \in \Val(X) \mid \exists c\in F, \delta>0 : 
p + \delta \cdot c \in G \}.
$$
%

We now prove a lemma which is close to being a counter-positive
of Lemma~\ref{lem:exit1}, except that it only applies to a certain 
portion of a \emph{convex} polyhedron.

\begin{lemma} \label{lem:exit2}
If a convex polyhedron $P$ is not bounded w.r.t.\ $\clos{\Flow(l)}$
then each point $P \cap \pospref{P}$ is not $l$-bounded.
\end{lemma}
%
Conversely, the set $P \setminus \pospref{P}$ is $l$-thin,
as may be easily verified from the definitions. \\
%
Next, we define the operator $\ru$ (for \emph{Remove Unbounded}) that,
given a polyhedron $G$, removes some convex regions of $G$ that are
not $l$-bounded, in such a way that the remaining set is $l$-bounded.
Let $B$ be the subset of $\conv{G}$ containing the convex polyhedra that
are bounded w.r.t. $\clos{\Flow(l)}$. We set
$$
\ru(G) = \bigcup_{P \in B} P \:\cup 
         \bigcup_{P \in \conv{G}\setminus B} \big( P \setminus \pospref{P} \big).
$$
%For a convex polyhedron $P$, define
%$\apostf{P} = \bigcap_{r\in\rays(F)} \postf{P}{r}$.
%Intuitively, $\apostf{P}$ contains the points that can be reached
%from $P$ through all directions of flow. 
%

\begin{proposition} \label{prop:ru-bipartite}
For all polyhedra $G$, and all $P \in \conv{\ru(G)}$,
either $P$ is bounded w.r.t. $\clos{\Flow(l)}$ or $P$ is $l$-thin.
\end{proposition}
%
The following results shows that two $l$-thin polyhedra
cannot be adjacent in the direction of flow.
%
\begin{lemma} \label{lem:thin-adjacency}
Let $L_1$ and $L_2$ be two $l$-thin polyhedra.
For all $p \in L_1$, $c \in \Flow(l)$ and $\delta >0$
there exists $0< \delta' \leq \delta$ such that $p + \delta c \not\in L_2$.
\end{lemma}
\begin{proof}
By contradiction, assume that there is $p \in L_1$, $c \in \Flow(l)$
and $\delta > 0$ such that for all $0 < \delta' \leq \delta$
it holds $p + \delta c \in L_2$.
Let $p_1 = p + \frac{\delta}{2} c$ and 
$p_2 = p + \delta c = p_1 + \frac{\delta}{2} c$.
We have that $p_1,p_2 \in L_2$, which contradicts the fact that
$L_2$ is thin w.r.t. $\Flow(l)$.
\qed
\end{proof}

\begin{lemma} \label{lem:boundary}
Let $G$ be a polyhedron and $G' = \ru(G)$.
For all $P \in \conv{G'}$, let $b$ be a convex polyhedron such that
$b \subseteq \bound(P, G'\setminus P)$ and $b$ is traversed by the flow.
We have that $b$ is bounded w.r.t. $\clos{\Flow(l)}$.
\end{lemma}
\begin{proof}
If $P$ is bounded w.r.t.\ $\clos{\Flow(l)}$, the result is obvious.
Otherwise, by Proposition~\ref{prop:ru-bipartite}, $P$ must be $l$-thin.
By Lemma~\ref{lem:thin-adjacency}, 
$P$ is not adjacent in the direction of flow 
to any other $l$-thin polyhedron in $\conv{G'}$.
Hence, $b$ may be partitioned into a finite set of sub-borders $b_i$,
where $b_i$ is a subset of the boundary between $P$ and another
convex polyhedron $P_i \in \conv{G'}$, such that $P_i$
is bounded w.r.t. $\clos{\Flow(l)}$.
Therefore, we obtain the thesis.
\qed
\end{proof}
%


\begin{lemma} \label{lem:remunbound}
Let $G$ be a polyhedron such that each $P \in \conv{G}$ is either
bounded w.r.t.\ $\clos{\Flow(l)}$ or $l$-thin.
Then, $G$ is $l$-bounded.
\end{lemma}
%
The following proposition summarizes the main properties of the $\ru$ operator
and it is a direct consequence of Lemmas~\ref{lem:remunbound} and~\ref{lem:exit2}.

\begin{proposition} \label{prop:remunbound}
For all polyhedra $G$, it holds:
\emph{(i)} $\ru(G)$ is $l$-bounded, and
\emph{(ii)} $\bounded_l(G) \subseteq \ru(G)$.
\end{proposition}

Given two polyhedra $U$ and $V$, define $\over$ as 
$\ru(\overline{U} \cap \overline{V})$.
The following lemma proves that $\over$ satisfies 
the assumptions of Theorem~\ref{thm:must}.
Hence, since $\over$ is easily computable from $U$ and $V$ using 
basic operations on polyhedra, we can compute $\rwamust_l(U,V)$ 
using equation~\eqref{eq:must} and Theorem~\ref{thm:may}.

\begin{lemma} \label{lem:over}
For all polyhedra $U$ and $V$, 
it holds $\rwamust_l(U,V) \setminus U \subseteq
\bounded_l(\overline{U} \cap \overline{V})$.
%(U \setminus V) \cup
%\remunbound(\overline{U} \cap \overline{V})$.
\end{lemma}
\begin{proof}{}
Let $u \in \rwamust_l(U,V) \setminus U$. By definition, $u \in \overline{V}$
and for all $f \in\adm(\pair{l, u})$ there exists $\delta\geq 0$ such that
$f(\delta) \in U$. Hence, the thesis.
\qed
\end{proof}


